Few-shot learning via tensor hallucination

Few-shot classification addresses the challenge of classifying examples given only limited labeled data. A powerful approach is to go beyond data augmentation, towards data synthesis. However, most of data augmentation/synthesis methods for few-shot classification are overly complex and sophisticated, e.g. training a wGAN with multiple regularizers or training a network to transfer latent diversities from known to novel classes. We make two contributions, namely we show that: (1) using a simple loss function is more than enough for training a feature generator in the few-shot setting; and (2) learning to generate tensor features instead of vector features is superior. Extensive experiments on miniImagenet, CUB and CIFAR-FS datasets show that our method sets a new state of the art, outperforming more sophisticated few-shot data augmentation methods.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

% \def\ceil#1{\lceil #1 \rceil}
% \def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% % Vectors
% \def\vzero{{\bm{0}}}
% \def\vone{{\bm{1}}}
% \def\vmu{{\bm{\mu}}}
% \def\vtheta{{\bm{\theta}}}
% \def\va{{\bm{a}}}
% \def\vb{{\bm{b}}}
% \def\vc{{\bm{c}}}
% \def\vd{{\bm{d}}}
% \def\ve{{\bm{e}}}
% \def\vf{{\bm{f}}}
% \def\vg{{\bm{g}}}
% \def\vh{{\bm{h}}}
% \def\vi{{\bm{i}}}
% \def\vj{{\bm{j}}}
% \def\vk{{\bm{k}}}
% \def\vl{{\bm{l}}}
% \def\vm{{\bm{m}}}
% \def\vn{{\bm{n}}}
% \def\vo{{\bm{o}}}
% \def\vp{{\bm{p}}}
% \def\vq{{\bm{q}}}
% \def\vr{{\bm{r}}}
% \def\vs{{\bm{s}}}
% \def\vt{{\bm{t}}}
% \def\vu{{\bm{u}}}
% \def\vv{{\bm{v}}}
% \def\vw{{\bm{w}}}
% \def\vx{{\bm{x}}}
% \def\vy{{\bm{y}}}
% \def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tex/conclusion-1.tex <==
\section{Conclusion}
\label{conclusion}
In table \ref{tab:sota}, Baseline and Baseline-KD represent the backbone trained only with equations \ref{eq:cls} and \ref{eq:kl} respectively. VF and TF represent our feature hallucinator trained with vector features and tensor features respectively. TF-ft represents our tensor feature hallucinator with fine-tuning applied at inference time. It is clear from our experiments that training tensor feature hallucinator is superior to a vector feature hallucinator. Also, it can be deduced that using this simple loss function of minimizing the mean squared error of the generated samples to their class prototypes can effectively train a few-shot hallucinator. Lastly we can claim to provide new state of the art performance in all every dataset and every setting outperforming all other few-shot data augmentation methods. It should be noted that the most impressive results are the comparisons with the methods using ResNet18 as a backbone since the backbone network architectures are exactly the same.

==> tex/exp-1.tex <==
\section{Experiments}
\label{experiments}
%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
%------------------------------------------------------------------------------

\subsection{Competitors}
We compare our method with the rest of the state of the art data augmentation methods for few-shot learning. Most of the data augmentation techniques use ResNet-18 as backbone embedding model, therefore in order to have fair comparisons between methods we also use the same network. %Since only \cite{DTN} provide publicly available official code, we adapted \cite{DTN} to our code to make objective comparisons. Since no official code is available for the rest of the state-of-the-art few-shot classification data-augmentation methods such as: \cite{AFHN, variationalFSL, Ideme, semanticAugmentation, VIFSL} we re-implemented the best data-augmentation method, AFHN \cite{AFHN} and compared it against our method, however this cannot be claimed to be an objective comparison since there might be small details in the code that were ommited from the paper. The methods \cite{AFHN, Ideme, semanticAugmentation} claim that they use the same pre-trained backbone provided from the code of \cite{semanticAugmentation}. It should be noted that \cite{AFHN} uses ReLU activation as the last activation in the encoder, however through our experiments we found it that better results are provided through using the Sigmoid activation function.

\subsection{Setup}

\paragraph{Datasets:}
We carry out experiments on three commonly used few-shot classication benchmark datasets, \emph{mini}Imagenet, CUB and Cifar-FS. Further details regarding each dataset are provided in section \ref{app:datasets}
\paragraph{Tasks:} We consider $N$-way, $K$-shot classification tasks with $N = 5$ randomly sampled novel classes and $K \in \{1, 5\}$ randomly selected examples per class for support set $S$, that is, $L = 5K$ examples in total. For the query set $Q$, we randomly sample $15$ additional examples per class, that is, $M = 75$ examples in total, which is the most common choice in the literature~\cite{tpn, learning2selftrain, transmatch}. \paragraph{Networks:} In order to obtain as fair comparisons as possible with previous data augmentation methods \cite{deltaencoder, semanticAugmentation, Ideme, AFHN}, we use ResNet18 for our embedding model. Our tensor feature hallucinator consists of a conditioner network and generator network. The conditioner network consists of two 2D convolutional layers, with a ReLU activation function in-between, a flattening module to convert the tensors into vectors and a linear layer. The generator network consists of an unflattening module to convert a vector input into a tensor followed by 3 transposed 2D convolutional layers with ReLU activation functions in-between the layers and a sigmoid activation function at the output of the last transposed 2D convolutional layer. In order to compare the performance of using tensor features instead of vector features we adapted our hallucinator accordingly. For the vector feature hallucinator as a conditioner network we use a two-layer fully-connected network  with a ReLU activation in-between the layers. The vector generator uses the same network architecture as the conditioner with an extra sigmoid activation function applied at the output of the last fully-connected layer. Further details regarding implementation details are provided in section \ref{app:implementations}


%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{adjustbox}{width=1\textwidth}
\setlength\tabcolsep{4pt}
\begin{tabular}{lccccccc}
\toprule
\Th{Method}                     & \Th{Backbone} & \mc{2}{\Th{\emph{mini}ImageNet}} & \mc{2}{\Th{CUB}} &  \mc{2}{\Th{cifar-FS}}\\  
                                                &               & 1-shot    & 5-shot & 1-shot    & 5-shot & 1-shot    & 5-shot\\ \midrule
Meta-GAN \cite{metaGAN}                          & ConvNet-4     & 52.71\ci{0.64} & 68.63\ci{0.67}  & - & - & - & -\\
Delta-Encoder$\dagger$ \cite{deltaencoder}                                   & VGG-16        & 59.90\cip     & 69.70\cip & 69.80\ci{0.46} & 82.60\ci{0.35} & 66.70\cip & 79.80\cip\\
SalNet \cite{salnet}                 & ResNet-101    & 62.22\ci{0.87}        & 77.95\ci{0.65} & - & - & - & -\\
DTN \cite{DTN}                                   & Resnet-12     & 63.45\ci{0.86} & 77.91\ci{0.62} & 72.00\cip & 85.10\cip & 71.50\cip & 82.80\cip\\ \midrule

%Baseline\cite{semanticAugmentation}$\dagger$    & ResNet-18     & 52.73          & 73.31 & - & - & - & -\\
Dual TriNet \cite{semanticAugmentation}          & ResNet-18     & 58.80\ci{1.37} & 76.71\ci{0.69} & 69.61\cip & 84.10\cip & 63.41\ci{0.64} & 78.43\ci{0.64}\\ 
IDeMe-Net \cite{Ideme}                           & ResNet-18     & 59.14\ci{0.86} & 74.63\ci{0.74} & - & - & - & -\\ 
AFHN \cite{AFHN}                                 & ResNet-18     & 62.38\ci{0.72} & 78.16\ci{0.56} & 70.53\ci{1.01} & 83.95\ci{0.63} & 68.32\ci{0.93} & 81.45\ci{0.87}\\
VI-Net \cite{VIFSL}                              & ResNet-18     & 61.05\cip & 78.60\cip & 74.76\cip & 86.84\cip & - & -\\ \midrule
Baseline                                     & ResNet-18     & 56.81\ci{0.81}    & 78.31\ci{0.59} & 67.14\ci{0.89} & 86.22\ci{0.50} & 65.71\ci{0.95} & 84.68\ci{0.61}\\
Baseline-KD                                       & ResNet-18     & 59.62\ci{0.85}     & 79.64\ci{0.62} & 70.85\ci{0.90} & 87.64\ci{0.48} & 69.15\ci{0.94} & 85.89\ci{0.59}\\
VF                          & ResNet-18     & 61.92\ci{0.85} & 77.02\ci{0.64}  & 75.25\ci{0.86} & 87.96\ci{0.48} & 72.60\ci{0.93} & 84.26\ci{0.67}\\
\textbf{TF(ours)}                                   & ResNet-18      & \textbf{64.25}\ci{0.85}     & 80.10\ci{0.61} & \textbf{75.83}\ci{0.91} & 88.17\ci{0.48} & 73.88\ci{0.87} & 85.92\ci{0.61}\\
\textbf{TF-ft(ours)}                                   & ResNet-18     & 63.92\ci{0.86}     & \textbf{80.41}\ci{0.60} & 75.39\ci{0.86} & \textbf{88.72}\ci{0.47} & \textbf{73.89}\ci{0.88} & \textbf{87.15}\ci{0.58}\\
%AFHN\cite{AFHN}*                                & ResNet-18     & 54.71     & 70.38 & - & - & - & -\\ 
%AFHN\cite{AFHN}$\_$sgm*                         & ResNet-18     & 58.17     & 72.44 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm*                         & ResNet-18     & 59.76     & 74.38 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm$\_$cr*                   & ResNet-18     & 58.97     & 75.44 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm$\_$cr+sca*               & ResNet-18     & 58.17     & 75.95 & - & - & - & -\\
%VAE$\_$cond                                     & ResNet-18     & 60.79     & 76.94 & - & - & - & -\\
%VAE$\_$cond+sca                                 & ResNet-18     & 59.62     & 76.50 & - & - & - & -\\
%AE$\_$cond$\_$triplet                           & ResNet-18     & 60.30     & 76.42 & - & - & - & -\\
%AE$\_$cond$\_$triplet+sca                       & ResNet-18     & 60.88     & 76.81 & - & - & - & -\\
%VAE$\_$cond$\_$triplet                          & ResNet-18     & 59.75     & 76.08 & - & - & - & -\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{6pt}
\caption{$\dagger$: Delta-encoder uses VGG-16 backbone for \emph{mini}ImageNet and cifar-FS and ResNet-18 backbone for CUB. VF is our feature hallucinator trained with vector features. TF is our tensor feature hallucinator and TF-ft is our tensor feature hallucinator followed by fine-tuning at inference time}
\label{tab:sota}
\end{table*}
%------------------------------------------------------------------------------

==> tex/intro-1.tex <==
\section{Introduction}
\label{intro}
Deep learning continuously keeps improving the state of the art performance in multiple different areas such as computer vision \cite{imagenet} and natural language understanding \cite{language}. However, even though the success of deep learning models is undeniable, a fundamental limitation of them is their dependence on large amounts of labeled data. This limitation inhibits the applicability of the state of the art deep learning techniques in real-world problems where the cost of annotating data is high and data can be scarce, i.e. rare species classification.

In order to address this limitation, the field of few-shot learning has attracted significant research interest in recent years. Multiple different lines of research have been proposed over the years to address the few-shot learning problem. One of the most common lines of research is meta-learning, addressing the problem of few-shot learning by leveraging training episodes that mimic a few-shot task by having small number of classes and limited number of samples per class. Meta-learning approaches can further be partitioned in optimization-based approaches that attempt to learn to update the learner's meta-parameters \cite{MAML, CAVIA, reptile, ravilstm}, metric-based approaches that attempt to learn a discriminative embedding space where samples from a novel task are easy to classify \cite{siamese, prototypical, relationnet, matchingNets} and model-based approaches that depend on specific model architectures to learn how to update the learner's parameters effectively \cite{santoro, metaNet}.

Beyond meta-learning methods, other approaches include methods that leverage the manifold structure of the data either by label propagation, embedding propagation or through the use of graph neural networks \cite{fewshotGNN1, fewshotGNN2, tpn, ilpc} and domain adaptation techniques that attempt to reduce the domain shifts between source and target domains \cite{domain_one, l2cluster}. Another line of research constitutes of data augmentation methods that attempt to tackle the data deficiency by augmenting the few-shot training dataset with extra samples \cite{AFHN, VIFSL, semanticAugmentation, Ideme, antoniou, metaGAN}.

Our work falls into the data augmentation category. We show that using a simple loss function to train a feature hallucinator can provide significant performance boost and outperform the current state of the art methods that use more complex and sophisticated methods such as: wGANS, VAEs and networks trained to transfer sample diversity. Also, to the best of our knowledge, we are the first to propose to generate tensor features instead of vector features in the few-shot setting.%These methods in general attempt to either train a generator or identify a way to augment the few-shot dataset during inference in time such that the classification performance is improved. However most of the proposed data augmentation techniques use sophisticated generators borrowed from the general deep learning literature. For example \cite{AFHN} trains a wGAN based feature hallucinator combined with two regularizer while \cite{VIFSL} trains a VAE model where the few labelled examples are used to infer the mean and variance of each class. \cite{DTN} to  transfer  latent  diversities  in order to combine them with support features to generate new features, \cite{Ideme} train a deformation network to fuse reference images with novel images. However, most of these methods follow sophisticated training regimes, such as training a wGAN, VAE, sampling reference images in order to train a generator successfully. In contrast in our work we simply show that using a very simple loss function is more than enough to train a feature hallucinator showing at the same time that there is no added benefit from using any complex training regime.

%Our contributions are summarized below:
%\begin{itemize}
%    \item We show that using a very simple loss function to train a feature hallucinator provides similar performance to sophisticated training regimes such as wGANs and VAEs.
%    \item To the best of our knowledge, we are the first to  propose to generate feature tensors instead of vector features in the few-shot setting, thus exploiting the spatial and structural properties of the feature tensors.
%    \item We achieve new state of the art results comparing all \emph{few-shot} data augmentation techniques.
%    \item We show that our method can be combined with other methods successfully
%\end{itemize}

==> tex/method-1.tex <==
\section{Method}
\label{sec:method}
\subsection{Problem formulation}
\label{sec:problem}

% Following the recent insights from~\cite{rfs}, we follow their formulation for the pre-training stage.

We assume access to a labelled dataset $D_{\base}$ with each example having a label in one of the classes in $C_{\base}$. This dataset is used to learn a parametrized mapping $f_{\theta}: \cX \to \real^d$ from an input space $\cX$ to a $d$-dimensional \emph{feature} or \emph{embedding} space. The knowledge acquired at representation learning is used to solve \emph{novel tasks}, assuming access to a dataset $D_{\novel}$ with each example being associated with one of the classes $C_{\novel}$, where $C_{\novel}$ is disjoint from $C_{\base}$. In \emph{few-shot classification}~\cite{matchingNets}, a novel task is defined by sampling a \emph{support set} $S$ from $D_{\novel}$, consisting of $N$ classes with $K$ labeled examples per class, for a total of $L \defn NK$ examples. Given the mapping $f$ and the support set $S$, the problem is to learn an $N$-way classifier that makes predictions on unlabeled \emph{queries} also sampled from $D_{\novel}$. 
% This may involve adapting $f$ or not. However, $K$ is small and the challenge is to avoid overfitting $S$. 
Queries are treated independently of each other, this is referred to as \emph{inductive inference}.

\subsection{Representation learning}
\label{sec:representation}
The goal of the \emph{representation learning} stage is to learn an embebbing model, $f_{\theta}$, that is transferable and can be applied to $D_{\novel}$ in order to extract expressive vector feature embeddings, $f_{\theta}^{GAP}: \cX \to \real^d$. The use of the superscript term $GAP$ represents global average pooling applied to the output tensors of the backbone network. We follow the recent training regime proposed from \cite{rfs} to train our embedding model and follow a two-stage training regime.
In the first stage, we train the embedding model, $f_{\theta}$, on dataset $D_{\base}$ using standard cross-entropy multi-class classification loss. In order to convert the extracted feature vectors to cross-entropy loss, we use a base classifier, $C_{\phi}$. The complete training loss for the first training stage is defined as:
\begin{equation}
    \{\theta, \phi \} = \arg\min_{\theta, \phi}\displaystyle\sum_{i = 1}^I L^{ce}_i(C_{\phi}(f_{\theta}^{GAP}(x_i)), y_i) + R(\phi)
\label{eq:cls}
\end{equation}

where $R$ is a regularization term, $L^{ce}$ is the standard cross-entropy loss term and $I$ is the total number of available samples in $D_{\base}$. In the second stage of the training regime, we adopt a self-distillation procedure, which is a form of knowledge distillation where the student and teacher models are identical in architecture. The trained embedding model from the first training stage serves as the teacher model and we distill the knowledge from it  into a new student model. The student model is trained using a weighted sum of: a) a cross-entropy loss between the predictions of the student model and the ground truth labels b) a Kullback-Leibler (KL) divergence term between the predictions of the student and the teacher models. The training loss for the second training stage is defined as:
\begin{equation}
    \theta' = \arg\min_{\theta'}\displaystyle\sum_{i = 1}^I(\alpha L^{ce}_i(C_{\phi'}(f_{\theta'}^{GAP}(x_i)), y_i) + R(\phi') + \beta KL(f_{\theta'}^{GAP}(x_i), f_{\theta}^{GAP}(x_i))
\label{eq:kl}
\end{equation}

where $\alpha$ and $\beta$ are scalar weights, $L^{ce}$ is the standard cross-entropy loss, $I$ is the total number of available samples in $D_{\base}$ and $KL$ is the KL divergence of the predictions between the student model, $f_{\theta'}$, and the teacher model, $f_{\theta}$. Also, $C_{\phi'}$ represents an untrained classifier and not the one trained at the first training stage.
\subsection{Feature tensor hallucinator}
We use the student model, $f_{\theta'}$, pre-trained using equation \ref{eq:kl} as our embedding network in order to train our tensor feature hallucinator.
The output from the embedding network is a tensor, $f_{\theta'}: \cX \to \real^{d\times h \times w}$, where $(d, h, w )$ represent the number of channels, height and width of the output tensor. %The most common procedure is to either flatten the tensor or use global average pooling and decrease the dimension to $\real^d$ as it was the case when we trained our embedding model in section \ref{sec:representation}.
All of the existing feature hallucination methods are trained using vector features, however this means that the vector features lose significant information of their spatial and structural properties. In contrast our tensor feature hallucinator is trained on the output tensors before global average pooling is applied and generates tensor features as well. Generating tensors instead of vectors provides the opportunity to use architectures such as convolutional layers to exploit the spatial and structural properties of tensors.

Our tensor feature hallucinator consists of two network modules: a conditioner network, $h_c$, and a generator network, $h_g$. The conditioner network's purpose is to leverage the prototype tensor of each class in order to aid the generator network to generate class-dependent samples. The prototype tensor of every class, $i$, which is used as the input to the conditioner is calculated by:
\begin{equation}
    p_i = \frac{1}{K}\displaystyle\sum_{j=1}^{K}f_{\theta'}(x_i^j)
\label{eq:proto}
\end{equation}
where $p_i$ is the prototype of class $i$ and $K$ is the total number of samples of class $i$. The output is simply a learnt mapping from the prototype tensor to the prototype class-conditional vector, $s_i = h_c(p_i)$. The generator network takes as input a sample from a Normal distribution, $z \sim \mathcal{N}(0, 1)$ and the output of the conditioner network, $s_i$, generating a class-conditional tensor feature from class $i$, $t_i = h_g(z, s_i)$.

\subsection{Training hallucinator}
We train our hallucinator using a meta-training regime in a similar way to \cite{AFHN, semanticAugmentation, deltaencoder}, training over a large number of few-shot episodes. At every iteration we sample a new episode where we randomly sample $N$ different classes from $D_{\base}$ and $K$ samples per class. We calculate the prototype of each class as defined from equation \ref{eq:proto} and pass it to the conditioner network to generate the prototype class-conditional vector $s_i$. We sample $M$ samples from a Normal distribution, $[z^m]^M_{m=1} \sim \mathcal{N}(0, 1)$. Using the $M$ samples and each prototype class-conditional vector $s_i$, we leverage our generator network to generate $M$ conditional tensor features per class $i$,  $[h_g(z^m, s_i)]_{m=1}^M$. We train our tensor hallucinator with the objective to minimize the mean squared error  (MSE) of all class conditional generated samples of class $i$, to their respective class prototype $p_i$ as defined below:
\begin{equation}
    \{c, g\} = \arg \min_{c, g} \frac{1}{MN}\displaystyle\sum_{i = 1}^N\displaystyle\sum_{m=1}^M (h_g(z^m, s_i) - p_i)^2
\end{equation}
where $N$ is the total number of classes per episode and $M$ the number of generated samples per class.
%\begin{equation}
%    \mathbf{V_i} = h_g(\mathbf{Z_i}, s_i)
%\label{eq:vi}
%\end{equation}
%where $\mathbf{V_i}$ are the $M$ generated samples of class $i$, $\mathbf{V_i} = [f_g(z^1_i, s_i), f_g(z^2_i, s_i), \dots, f_g(z^M_i, s_i)]$




\subsection{Few-shot classification}
At inference time, given a few-shot learning task with a support set, $S$, of $N$ unique classes with $K$ examples per class we calculate the tensor feature of each sample using our trained backbone network, $f_{\theta'}$. Using the tensor features we calculate the prototype, $p_i$, of every class $i$ as defined from equation \ref{eq:proto} and using our trained tensor feature hallucinator we generate $M$ class-conditioned samples for every class. We augment the support set, $S$, by combining all the support samples with the generated samples, therefore for each class we have $\{K+M\}$ support samples. We apply global average pooling to both augmented support tensor features and query tensor features and calculate the vector class prototypes using the augmented support set. Lastly we classify each query simply to the class that its class prototype is closer. At inference time, we use vector instead of tensor features to classify queries since experimentally the performance was superior.%It should be noted that at the last stage of he few-shot classification procedure we used vector features instead of tensors for classifying the query samples since experimentally the performance was superior.% and re-calculate the class prototypes using the augmented support set. %Lastly for every query sample we calculate its tensor feature, apply global averaging pooling to both the query tensor feature and the class prototypes and classify the query simply to the class that its class prototype is closer. Note that at inference time rather than calculating each query using its feature tensor and the tensor prototypes, we perform global average pooling since there is negligible difference in classification performance.


==> tex/related.tex <==
%\section{Related work}
%\label{related}
%Multiple different lines of research have been proposed over the years to address the few-shot learning problem. One of the more common lines of research is meta-learning, where they tackle the problem of few-shot learning by the concept of "learning to learn" leveraging training episodes that mimic the few-shot task by having small number of classes and limited number of samples per class. Meta-learning approaches can further be partitioned in optimization-based approaches that attempt to learn to update the learner's model meta-parameters \cite{MAML, CAVIA, reptile, ravilstm}, metric-based approaches that attempt to learn a discriminative embedding space where samples from a novel task are easy to classify \cite{siamese, prototypical, relationnet, matchingNets} and model-based approaches that depend on specific model architectures to learn how to update the learner's parameters effectively \cite{santoro, metaNet}.
%Beyond meta-learning methods, other approaches include methods that leverage the manifold structure of the data either by label propagation or embedding propagation or through the use of graph neural networks \cite{fewshotGNN1, fewshotGNN2, tpn, ilpc} and domain adaptation techniques that attempt to reduce the domain shifts between source and target domain domains \cite{domain_one, l2cluster}. Another line of research constitutes of data augmentation methods that attempt to tackle the data deficiency by effectively providing more training data \cite{AFHN, VIFSL, semanticAugmentation, Ideme, antoniou, metaGAN}.
